A Taxonomy of Recurrent Learning Rules

Backpropagation through time (BPTT) is the de facto standard for training recurrent neural networks (RNNs), but it is non-causal and non-local. Real-time recurrent learning is a causal alternative, but it is highly inefficient. Recently, e-prop was proposed as a causal, local, and efficient practical alternative to these algorithms, providing an approximation of the exact gradient by radically pruning the recurrent dependencies carried over time. Here, we derive RTRL from BPTT using a detailed notation bringing intuition and clarification to how they are connected. Furthermore, we frame e-prop within in the picture, formalising what it approximates. Finally, we derive a family of algorithms of which e-prop is a special case.

==> figures/name_.tex <==
\begin{itemize}
    \item 1) \textbf{Explicit recurrences:} Compute \smash{$\dv{\loss}{\ovar^{t}_j}$} using the recursive definition given by the explicit recurrences (both self-explicit and inter-explicit, see Fig. \ref{fig:EandIandB}A):
    
    \begin{equation}\label{eqdedz}
        \begin{split}
    \dv{\loss}{\ovar^{t}_j} &= \cdv{ \loss}{ \ovar^{t}_j} +  \dv{\loss}{\ovar^{t+1}_j} \cdv{ \ovar^{t+1}_j}{ \hvar_j^{t+1}} \cdv{ \hvar_j^{t+1}}{ \ovar_j^{t}} + \sum_{k \neq j} \dv{\loss}{\ovar^{t+1}_k} \cdv{ \ovar^{t+1}_k}{ \hvar_k^{t+1}} \cdv{ \hvar_k^{t+1}}{ \ovar_j^{t}}  = \\
    &= \cdv{ \loss}{ \ovar^{t}_j} + \sum_k \dv{\loss}{\ovar^{t+1}_k} \cdv{ \ovar^{t+1}_k}{ \hvar_k^{t+1}} \cdv{ \hvar_k^{t+1}}{ \ovar_j^{t}}
    \end{split}
    \end{equation}
    
    \item 2) \textbf{Implicit recurrence:} Compute \smash{$\dv{\loss}{\hvar^{t}_j}$} using the value of the previous step and the recursive definition given by the implicit recurrence (see Fig.\ref{fig:EandIandB}B):
    
    \begin{equation}\label{eqdedh}
    \dv{\loss}{\hvar^{t}_j} = \dv{\loss}{\ovar^{t}_j} \cdv{ \ovar^{t}_j}{ \hvar_j^{t}} + \dv{\loss}{\hvar^{t+1}_j}\cdv{ \hvar_j^{t+1}}{ \hvar_j^{t}}
    \end{equation}
    
    \item 3) \textbf{BPTT:} Finally compute \smash{$\dv{\loss}{W_{ji}}$} using the values of the previous two steps (Fig.\ref{fig:EandIandB}C):
    
    \begin{equation}\label{eqg1}
    \dv{\loss}{W_{ji}} = \sum_{t} \dv{\loss}{\hvar_j^{t}} \cdv{ \hvar^{t}_j}{ W_{ji}}
    \end{equation}
\end{itemize}

The existence of this recurrences makes BPTT present the following biological plausiblity problems \cite{Marblestone2016, Bellec2019}:

\begin{itemize}
    \item \textbf{Non-locality}. Due to the inter-explicit recurrence, we need to take into account how the current strength of the synapse $ji$ affects the future synapse: \smash{$\cdv{ \hvar^{t+1}_k}{ \ovar^t_j}$} for all $k \neq j$ (see Eq \ref{eqdedz}). This means that to compute the weight change for synapse magnitude $W_{ji}$ we need information of synapse $\ovar^{t}_j \rightarrow \hvar^{t+1}_k$ for all $k$. Even worse, this chain of dependencies continues at each time step, such that at the next time step we needed information of synapse $\ovar^{t+1}_k \rightarrow \hvar^{t+2}_q$ for all $q$ (including $q \neq j$) and so forth. Therefore the algorithm requires all synapses to be connected with every neuron. This is not very biologically plausible, and its been coined the ``spatial credit assignment'' problem. The contraposition would be a \textbf{local} algorithm that does not require messages passing from every neuron to every synapse to compute the gradients, but rather only need information close to the given synapse.
    \item \textbf{Non-causality}. Due to the three kind of recurrences shown before we need to take into account all the gradients in the future (the same way as current layer computations need to use the gradients of posterior layers in feed-forward architectures). This leads to two restrictions:
    \begin{itemize}
        \item \emph{Locking:} We need, across all future time-steps, to compute the values of the variables (update locking) and the gradients (backwards locking) before computing the current gradient \cite{Czarnecki2017}. This requires the system to have a multiplexing mechanism for changing between inference and learning phases, as well as to stop inference while it is learning. Both this aspects seem problematic for biological systems.
        \item \emph{Memory storage:} All the values of all the variables across time have to be saved during the inference phase to be used while computing the gradients. This is not biologically plausible since it requires a huge memory overhead ($O(nT)$ with $n$ neurons and $T$ time steps), storing many values in an organised manner. This problem has been coined the ``temporal credit assignment'' problem.
    \end{itemize}
    The contraposition would be a \textbf{causal} algorithm, that at each time step would only need information from previous and current activity to compute the current gradient. Therefore, it could do it at each time step (\textbf{online}) and while the inference is running.
\end{itemize}

These problems are also of great importance for the implementation of BPTT in neuromorphic hardware \cite{Zenke2020}. 

An important point to make is what happens with the gradient \smash{$\cdv{ \ovar^t_j}{ \hvar^t_j}$} since the function that defines $\ovar^t_j$ from $v^t_j \in \hvar^t_j$ is the Heaviside function, which has no derivative at $v^t_j = v_{th}$ and is constantly $0$ elsewhere. To solve this, in the computation of the gradient we use a different derivative. These derivatives are called ``surrogate gradients'' and there are many options that work well in practice \cite{Zenke2021}.

\section{RTRL}

\texbf{RTRL} (Real Time Recurrent Learning) is a causal learning algorithm (can be implemented as an online learning algorithm) that computes exactly the same gradient as BPTT but at the cost of being more computationally expensive. 

Let's derive the equation for RTRL for our computational graph in Fig. \ref{fig:CompGraphColors}. 

The idea is that we start with BPTT Eq \ref{eqg1}:
\begin{equation}\label{eqg12}
    \dv{\loss}{W_{ji}} = \sum_{t'} \dv{\loss}{\hvar_j^{t'}} \cdv{ \hvar^{t'}_j}{ W_{ji}}
\end{equation}

and we want to reexpress the gradients that connect the computation with future gradients to achieve a causal algorithm. These correspond to the implicit, inter-explicit and sef-explicit recurrence.

\subsection{Reexpressing implicit recurrence}
\label{sect:ReexImplicitRec}

First, we focus on reexpressing the implicit recurrence gradient \smash{$\cdv{ \hvar_j^{t'+1}}{ \hvar_j^{t'}}$}. For this we plug in the equation of implicit recurrence Eq \ref{eqdedh} in Eq \ref{eqg12}:

\begin{equation}
\begin{split}
    \dv{\loss}{W_{ji}} =& \sum_{t'} \left( \dv{\loss}{\ovar^{t'}_j} \cdv{ \ovar^{t'}_j}{ \hvar_j^{t'}} + \dv{\loss}{\hvar^{t'+1}_j}\cdv{ \hvar_j^{t'+1}}{ \hvar_j^{t'}} \right) \cdv{ \hvar^{t'}_j}{ W_{ji}} = \\
    =&\sum_{t'} \left( \dv{\loss}{\ovar^{t'}_j} \cdv{ \ovar^{t'}_j}{ \hvar_j^{t'}} + \left( \dv{\loss}{\ovar^{t'+1}_j} \cdv{ \ovar^{t'+1}_j}{ \hvar_j^{t'+1}} + (\dvotsi) \cdv{ \hvar_j^{t'+2}}{ \hvar_j^{t'+1}} \right) \cdv{ \hvar_j^{t'+1}}{ \hvar_j^{t'}} \right) \cdv{ \hvar^{t'}_j}{ W_{ji}} = \\
    =&\sum_{t'}\sum_{t \geq t'} \dv{\loss}{\ovar^t_j} \cdv{ \ovar^t_j}{ \hvar^t_j} \cdv{ \hvar^t_j}{ \hvar^{t-1}_j} \dvotsi \cdv{ \hvar^{t'+1}_j}{ \hvar^{t'}_j} \cdv{ \hvar^{t'}_j}{ W_{ji}}
\end{split}
\end{equation}

This formula is non-causal since it requires future gradients (for each $t'$ we sum products of gradients with factors starting from $t \geq t'$). To make it causal, we do a change of indices as follows:
\begin{equation}\label{eqichang}
\begin{split}
    \dv{\loss}{W_{ji}} =& \sum_{t'}\sum_{t \geq t'} \dv{\loss}{\ovar^t_j} \cdv{ \ovar^t_j}{ \hvar^t_j} \cdv{ \hvar^t_j}{ \hvar^{t-1}_j} \dvotsi \cdv{ \hvar^{t'+1}_j}{ \hvar^{t'}_j} \cdv{ \hvar^{t'}_j}{ W_{ji}} = \\
    =&\sum_t \dv{\loss}{\ovar^t_j} \cdv{ \ovar^t_j}{ \hvar^t_j} \sum_{t' \leq t} \cdv{ \hvar^t_j}{ \hvar^{t-1}_j} \dvotsi \cdv{ \hvar^{t'+1}_j}{ \hvar^{t'}_j}  \cdv{ \hvar^{t'}_j}{ W_{ji}}
\end{split}
\end{equation}

\begin{figure}
\includegraphics[width=\textwidth]{figures/iet.png} 
\caption{Computational graph for the implicit variable $e^t_{ji}$ with $t'=0$.}
\label{fig:IET}
\end{figure}

Now we can define the \emph{implicit variable} $ \pmb{\epsilon}^t_{ji}$ (see Fig. \ref{fig:IET}):

\begin{equation}\label{eqiet}
     \pmb{\epsilon}_{ji}^t = \sum_{t' \leq t} \cdv{ \hvar^t_j}{ \hvar^{t-1}_j} \dvotsi \cdv{ \hvar^{t'+1}_j}{ \hvar^{t'}_j}  \cdv{ \hvar^{t'}_j}{ W_{ji}}
\end{equation}

It represents how the hidden variables of neuron $j$ (voltage but also e.g. threshold adaptation) have been affected by the synapse weight $W_{ji}$ through time. I.e. taking into account also the implicit recurrence: how the hidden variables at previous time steps have affected the variables at the current time step. This value is specific for each synapse and therefore it is local.

Importantly, there is a recursive relation to this variable that allows it to be updated at each time step. Therefore it is also causal:

\begin{equation}
     \pmb{\epsilon}_{ji}^t = \cdv{ \hvar^t_j}{ \hvar^{t-1}_j}  \pmb{\epsilon}^{t-1}_{ji} + \cdv{ \hvar^t_j}{ W_{ji}}
\end{equation}

To simplify notation, we define the \emph{implicit eligibility trace} from the implicit variable as

\begin{equation}
    e^t_{ji} = \cdv{ \ovar^{t}_j}{ \hvar^{t}_j} \pmb{\epsilon}^t_{ji}
\end{equation} 

Since \smash{$\cdv{ \ovar^{t}_j}{ \hvar^{t}_j}$} is causal and local, and so is the implicit variable $\pmb{\epsilon}^t_{ji}$, then the implicit eligibility trace $e^t_{ji}$ is also causal and local.

With all of this, BPTT Eq \ref{eqg12} has become (substituting Eq \ref{eqiet} in Eq \ref{eqichang}) the following (see Fig. \ref{fig:eprop}A): 

\begin{equation} \label{eqg2}
    \dv{\loss}{W_{ji}} = \sum_{t} \dv{\loss}{\ovar^{t}_j} \cdv{ \ovar^{t}_j}{ \hvar^{t}_j}  \pmb{\epsilon}_{ji}^{t} = \sum_{t} \dv{\loss}{\ovar^{t}_j} e^{t}_{ji}
\end{equation} 

Even though $e^t_{ji}$ is local and causal, this equation as a whole in general is not, since the factor \smash{$\dv{\loss}{\ovar^{t}_j}$} still includes explicit recurrences. In Chapter \ref{chap:e-prop} we will see that \emph{e-prop} will simply ignore these recurrences to solve this problem.

\begin{figure}
\includegraphics[width=\textwidth]{figures/Eeprop.png} 
\caption{Computational graph for A) BPTT reexpressed with implicit elegibility trace (Eq \ref{eqg2}) B) symmetric e-prop.}
\label{fig:eprop}
\end{figure}

\subsection{Reexpressing explicit recurrences}

Now we focus on reexpressing the explicit recurrences' gradient \smash{$\cdv{ \hvar_k^{t+1}}{ \ovar_j^{t}}$} with $k = j$ (self-explicit) and $k \neq j$ (inter-explicit). We do it in a complete analogous form as before. First, we plug in the equation of explicit recurrences Eq \ref{eqdedz} into what we obtained in the last step, Eq \ref{eqg2}:

\begin{equation}
\begin{split}
    \dv{\loss}{W_{ji}} =& \sum_{t'} \left(\cdv{ \loss}{ \ovar^{t'}_j} + \sum_k \dv{\loss}{\ovar^{t'+1}_k} \cdv{ \ovar^{t'+1}_k}{ \hvar_k^{t'+1}} \cdv{ \hvar_k^{t'+1}}{ \ovar_j^{t'}} \right) e^{t'}_{ji} = \\
    =& \sum_{t'} \left(\cdv{ \loss}{ \ovar^{t'}_j} + \sum_k \left(\cdv{ \loss}{ \ovar^{t'+1}_k} + \sum_{k'} (\dvotsi) \cdv{ \ovar^{t'+2}_{k'}}{ \hvar_{k'}^{t'+2}} \cdv{ \hvar_{k'}^{t'+2}}{ \ovar_k^{t'+1}} \right)  \cdv{ \ovar^{t'+1}_k}{ \hvar_k^{t'+1}} \cdv{ \hvar_k^{t'+1}}{ \ovar_j^{t'}} \right) e^{t'}_{ji} = \\
    =& \sum_{t'} \sum_{t \geq t'} \sum_{k^{(t'+1)},..,k^t} \cdv{ \loss}{ \ovar^t_{k^t}}  \cdv{ \ovar^t_{k^t}}{ \hvar_{k^t}^t} \cdv{ \hvar_{k^{t}}^t}{ \ovar_{k^{(t-1)}}^{t-1}} \dvotsi \cdv{ \ovar^{t'+1}_{k^{(t'+1)}}}{ \hvar_{k^{(t'+1)}}^{t'+1}} \cdv{ \hvar_{k^{(t'+1)}}^{t'+1}}{ \ovar_j^{t'}} e^{t'}_{ji}
\end{split}
\end{equation}

The notation starts to get cumbersome but the intuitive idea is that for every time step $t$ we consider the influence on the synapse of a neuron $k^t$  by any presynaptic neuron $k^{(t-1)}$ with the factor $\cdv{ \ovar^t_{k^t}}{ \hvar_{k^t}^t} \cdv{ \hvar_{k^{t}}^t}{ \ovar_{k^{(t-1)}}^{t-1}}$. Since in general any neuron at time $t$ can be influenced by neuron $j$ at time $t'$ through any path of synapses, we need to summate across all possible combination of neurons $k^{(t'+1)},..,k^t$.

As before we change the time indeces and reorganise to allow for causality,
\begin{equation}\label{eqpchang}
\begin{split}
    \dv{\loss}{W_{ji}} =& \sum_{t'} \sum_{t \geq t'} \sum_{k^{(t'+1)},..,k^t} \cdv{ \loss}{ \ovar^t_{k^t}}  \cdv{ \ovar^t_{k^t}}{ \hvar_{k^t}^t} \cdv{ \hvar_{k^{t}}^t}{ \ovar_{k^{t-1}}^{(t-1)}} \dvotsi \cdv{ \ovar^{t'+1}_{k^{(t'+1)}}}{ \hvar_{k^{(t'+1)}}^{t'+1}} \cdv{ \hvar_{k^{(t'+1)}}^{t'+1}}{ \ovar_j^{t'}} e^{t'}_{ji} = \\
    =& \sum_t \sum_{k^t} \cdv{ \loss}{ \ovar^t_{k^t}} \cdv{ \ovar^t_{k^t}}{ \hvar_{k^t}^t} \sum_{t' \leq t} \sum_{k^{(t'+1)},..,k^{(t-1)}} \cdv{ \hvar_{k^t}^t}{ \ovar_{k^{(t-1)}}^{t-1}} \cdv{ \ovar^{t-1}_{k^{(t-1)}}}{ \hvar_{k^{(t-1)}}^{t-1}} \dvotsi \cdv{ \hvar_{k^{(t'+1)}}^{t'+1}}{ \ovar_j^{t'}} e^{t'}_{ji}
\end{split}
\end{equation}

Now we can define the \emph{recurrence variabl\loss} $ \pmb{\alpha}^{t,r}_{ji}$ which includes inside the implicit elegibility trace $ e^t_{ji}$ but also the explicit recurrences: 
\begin{equation}\label{eqpet}
     \pmb{\alpha}^{t,r}_{ji} = \sum_{t' \leq t} \sum_{k^{(t'+1)},..,k^{(t-1)}} \cdv{ \hvar_r^t}{ \ovar_{k^{(t-1)}}^{t-1}} \cdv{ \ovar^{t-1}_{k^{(t-1)}}}{ \hvar_{k^{(t-1)}}^{t-1}} \dvotsi \cdv{ \hvar_{k^{(t'+1)}}^{t'+1}}{ \ovar_j^{t'}} e^{t'}_{ji}
\end{equation}

Once again, importantly, we have a recursive equation for computing the partial recurrence variable, making it a causal magnitude. However, it is not local in an equivalent way as BPTT is not: each synapse $ji$ requires to store a variable representing how the activation in the past of any other neuron $r$ would affect its computation, even if $r \neq j,i$. The recursive computation requires of the summation of the recurrence variables of all the neurons requiring also non-local communication:

\begin{equation}
     \pmb{\alpha}^{t,r}_{ji} =  \sum_{k} \cdv{ \hvar^t_r}{ \ovar_{k}^{t-1}} \cdv{ \ovar_{k}^{t-1}}{ \hvar_{k}^{t-1}} \pmb{\alpha}^{t-1,k}_{ji} + e^t_{ji}
\end{equation}

To simplify notation, we define the \emph{recurrence elegibility trace}
\begin{equation}
    a_{ji}^{t,r} = \cdv{ \ovar^t_{r}}{ \hvar_{r}^t} \pmb{\alpha}^{t,r}_{ji}
\end{equation}

Since \smash{$\cdv{ \ovar^t_{r}}{ \hvar_{r}^t}$} is causal and local, but the recurrence variable $\pmb{\alpha}^{t,r}_{ji}$ is causal but non-local, then the recurrence eligibility trace $a^{t,r}_{ji}$ is also causal but non-local.

Eq \ref{eqg2} transforms into (by substituting Eq \ref{eqpet} into Eq \ref{eqpchang}) the final equation for RTRL: 

\begin{equation}\label{eqRTRL}
    \dv{\loss}{W_{ji}} = \sum_{t} \sum_{k} \cdv{ \loss}{ \ovar^{t}_{k}} \cdv{ \ovar^t_{k}}{ \hvar_{k}^t}  \pmb{\alpha}^{t,k}_{ji} = \sum_{t} \sum_{k} \cdv{ \loss}{ \ovar^{t}_{k}} a_{ji}^{t,k}
\end{equation}

\subsection{Reexpressing explicit recurrences (CORRECT?)}

Now we focus on reexpressing the explicit recurrences' gradient \smash{$\cdv{ \hvar_k^{t+1}}{ \ovar_j^{t}}$} with $k = j$ (self-explicit) and $k \neq j$ (inter-explicit). We do it in a complete analogous form as before. First, we plug in the equation of explicit recurrences Eq \ref{eqdedz} into what we obtained in the last step, Eq \ref{eqg2}:

\begin{equation}
\begin{split}
    \dv{\loss}{W_{ji}} =& \sum_{t'} \left(\cdv{ \loss}{ \ovar^{t'}_j} + \sum_k \dv{\loss}{\ovar^{t'+1}_k} \cdv{ \ovar^{t'+1}_k}{ \hvar_k^{t'+1}} \cdv{ \hvar_k^{t'+1}}{ \ovar_j^{t'}} \right) e^{t'}_{ji} = \\
    =& \sum_{t'} \left(\cdv{ \loss}{ \ovar^{t'}_j} + \sum_k \left(\cdv{ \loss}{ \ovar^{t'+1}_k} + \sum_{k'} (\dvotsi) \cdv{ \ovar^{t'+2}_{k'}}{ \hvar_{k'}^{t'+2}} \cdv{ \hvar_{k'}^{t'+2}}{ \ovar_k^{t'+1}} \right)  \cdv{ \ovar^{t'+1}_k}{ \hvar_k^{t'+1}} \cdv{ \hvar_k^{t'+1}}{ \ovar_j^{t'}} \right) e^{t'}_{ji} = \\
    =& \sum_{t'} \sum_{t \geq t'} \sum_{k^{(t'+1)},..,k^t} \cdv{ \loss}{ \ovar^t_{k^t}}  \cdv{ \ovar^t_{k^t}}{ \hvar_{k^t}^t} \cdv{ \hvar_{k^{t}}^t}{ \ovar_{k^{(t-1)}}^{t-1}} \dvotsi \cdv{ \ovar^{t'+1}_{k^{(t'+1)}}}{ \hvar_{k^{(t'+1)}}^{t'+1}} \cdv{ \hvar_{k^{(t'+1)}}^{t'+1}}{ \ovar_j^{t'}} e^{t'}_{ji}
\end{split}
\end{equation}

The notation starts to get cumbersome but the intuitive idea is that for every time step $t$ we consider the influence on the synapse of a neuron $k^t$  by any presynaptic neuron $k^{(t-1)}$ with the factor $\cdv{ \ovar^t_{k^t}}{ \hvar_{k^t}^t} \cdv{ \hvar_{k^{t}}^t}{ \ovar_{k^{(t-1)}}^{t-1}}$. Since in general any neuron at time $t$ can be influenced by neuron $j$ at time $t'$ through any path of synapses, we need to summate across all possible combination of neurons $k^{(t'+1)},..,k^t$.

As before we change the time indeces and reorganise to allow for causality,
\begin{equation}\label{eqpchang}
\begin{split}
    \dv{\loss}{W_{ji}} =& \sum_{t'} \sum_{t \geq t'} \sum_{k^{(t'+1)},..,k^t} \cdv{ \loss}{ \ovar^t_{k^t}}  \cdv{ \ovar^t_{k^t}}{ \hvar_{k^t}^t} \cdv{ \hvar_{k^{t}}^t}{ \ovar_{k^{t-1}}^{(t-1)}} \dvotsi \cdv{ \ovar^{t'+1}_{k^{(t'+1)}}}{ \hvar_{k^{(t'+1)}}^{t'+1}} \cdv{ \hvar_{k^{(t'+1)}}^{t'+1}}{ \ovar_j^{t'}} e^{t'}_{ji} = \\
    =& \sum_t \sum_{k^t} \cdv{ \loss}{ \ovar^t_{k^t}} \cdv{ \ovar^t_{k^t}}{ \hvar_{k^t}^t} \sum_{t' \leq t} \sum_{k^{(t'+1)},..,k^{(t-1)}} \cdv{ \hvar_{k^t}^t}{ \ovar_{k^{(t-1)}}^{t-1}} \cdv{ \ovar^{t-1}_{k^{(t-1)}}}{ \hvar_{k^{(t-1)}}^{t-1}} \dvotsi \cdv{ \hvar_{k^{(t'+1)}}^{t'+1}}{ \ovar_j^{t'}} e^{t'}_{ji}
\end{split}
\end{equation}

Now we can define the \emph{recurrence variabl\loss} $ \pmb{\alpha}^{t,r}_{ji}$ which includes inside the implicit elegibility trace $ e^t_{ji}$ but also the explicit recurrences: 
\begin{equation}\label{eqpet}
     \pmb{\alpha}^{t,r}_{ji} = \sum_{t' \leq t} \sum_{k^{(t'+1)},..,k^{(t-1)}} \cdv{ \hvar_r^t}{ \ovar_{k^{(t-1)}}^{t-1}} \cdv{ \ovar^{t-1}_{k^{(t-1)}}}{ \hvar_{k^{(t-1)}}^{t-1}} \dvotsi \cdv{ \hvar_{k^{(t'+1)}}^{t'+1}}{ \ovar_j^{t'}} e^{t'}_{ji}
\end{equation}

Once again, importantly, we have a recursive equation for computing the partial recurrence variable, making it a causal magnitude. However, it is not local in an equivalent way as BPTT is not: each synapse $ji$ requires to store a variable representing how the activation in the past of any other neuron $r$ would affect its computation, even if $r \neq j,i$. The recursive computation requires of the summation of the recurrence variables of all the neurons requiring also non-local communication:

\begin{equation}
     \pmb{\alpha}^{t,r}_{ji} =  \sum_{k} \cdv{ \hvar^t_r}{ \ovar_{k}^{t-1}} \cdv{ \ovar_{k}^{t-1}}{ \hvar_{k}^{t-1}} \pmb{\alpha}^{t-1,k}_{ji} + e^t_{ji}
\end{equation}

To simplify notation, we define the \emph{recurrence elegibility trace}
\begin{equation}
    a_{ji}^{t,r} = \cdv{ \ovar^t_{r}}{ \hvar_{r}^t} \pmb{\alpha}^{t,r}_{ji}
\end{equation}

Since \smash{$\cdv{ \ovar^t_{r}}{ \hvar_{r}^t}$} is causal and local, but the recurrence variable $\pmb{\alpha}^{t,r}_{ji}$ is causal but non-local, then the recurrence eligibility trace $a^{t,r}_{ji}$ is also causal but non-local.

Eq \ref{eqg2} transforms into (by substituting Eq \ref{eqpet} into Eq \ref{eqpchang}) the final equation for RTRL: 

\begin{equation}\label{eqRTRL}
    \dv{\loss}{W_{ji}} = \sum_{t} \sum_{k} \cdv{ \loss}{ \ovar^{t}_{k}} \cdv{ \ovar^t_{k}}{ \hvar_{k}^t}  \pmb{\alpha}^{t,k}_{ji} = \sum_{t} \sum_{k} \cdv{ \loss}{ \ovar^{t}_{k}} a_{ji}^{t,k}
\end{equation}

Therefore we have now a gradient computation algorithm that is causal but still non-local. e-prop is an algorithm that is both causal and local.

\section{Definition}

To derive the synaptic rules for \textbf{e-prop} (Eligibility propagation) we start from Eq \ref{eqg2}, where we had expressed BPTT with the implicit eligibility trace (Fig. \ref{fig:eprop}A):

\begin{equation}\label{eqg3}
    \dv{E}{W_{ji}} = \sum_{t} \dv{E}{\ovar^{t}_j} e^t_{ji}
\end{equation} 

Since $e^t_{ji}$ is causal and local, it is up for \smash{$\dv{E}{\ovar^{t}_j}$} to determine if the whole algorithm also is. However, as we have seen in explicit recurrence equation Eq \ref{eqdedz}, \smash{$\dv{E}{\ovar^{t}_j}$} is neither causal nor local:

\begin{equation}\label{eqdedz2}
    \dv{E}{\ovar^{t}_j} = \cdv{\loss}{ \ovar^{t}_j} + \sum_k \dv{E}{\ovar^{t+1}_k} \cdv{ \ovar^{t+1}_k}{ \hvar_k^{t+1}} \cdv{ \hvar_k^{t+1}}{ \ovar_j^{t}}
\end{equation}

Finding a recursive expression does, as we have seen, make the resulting RTRL method (Eq \ref{eqRTRL}) causal, but not local. 

\emph{e-prop} solves this by just approximating \smash{$\dv{E}{\ovar^{t}_j}$}. 


\section{Symmetric e-prop}
\subsection{Approximation}

From Eq \ref{eqdedz2} we conclude that a good approximation is \smash{$\dv{E}{\ovar^{t}_j} \approx \cdv{\loss}{ \ovar^{t}_j}$}, ignoring the explicit recurrence of the model. In this case, if the architecture is a single forward layer, this is not an approximation but an exact computation. This leads, from Eq \ref{eqg3}, to the following (see Fig.\ref{fig:eprop}B):

\begin{equation}
    \dv{E}{W_{ji}} \approx \sum_{t} \cdv{\loss}{ \ovar^{t}_j} e^t_{ji}
\end{equation} 

If we use this approximation of the gradient for a vanilla gradient descent learning rule, we get \textbf{symmetric e-prop}:

\begin{equation} \label{eqseprop}
    \Delta W^{rec}_{ji} = - \eta \sum_t \cdv{\loss}{ \ovar^t_j}e^t_{ji}
\end{equation}

\subsection{Feed-forward restriction}
\label{sect:FFrest}

This approximation however does not come without consequences. Consider the separation of the explicit recurrence into the self-explicit and inter-explicit recurrence as in Eq \ref{eqdedz}:
\begin{equation}
    \sum_k \dv{E}{\ovar^{t+1}_k} \cdv{ \ovar^{t+1}_k}{ \hvar_k^{t+1}} \cdv{ \hvar_k^{t+1}}{ \ovar_j^{t}} = \dv{E}{\ovar^{t+1}_j} \cdv{ \ovar^{t+1}_j}{ \hvar_j^{t+1}} \cdv{ \hvar_j^{t+1}}{ \ovar_j^{t}} + \sum_{k \neq j} \dv{E}{\ovar^{t+1}_k} \cdv{ \ovar^{t+1}_k}{ \hvar_k^{t+1}} \cdv{ \hvar_k^{t+1}}{ \ovar_j^{t}}
\end{equation}

Ignoring the self-explicit recurrence ($\ovar^t_j \nrightarrow \hvar^{t+1}_j$) is not a problem (see Fig. \ref{fig:eprop}B, yellow line). Thanks to the implicit eligibility trace $e^t_{ji}$ information on how the synaptic weight affects the hidden variables at time $t$ can be taken into account when computing the influence on the loss function of the synaptic value of the same neuron at time $t+1$. Furthermore, many architectures do not use self-synapses, making this approximation thinner.

However, ignoring the inter-explicit recurrence ($\ovar^t_j \nrightarrow \hvar^{t+1}_k$) comes with an important constraint on the architecture. If a neuron $j$ does not directly influence the loss (it is not connected to readout neurons, $\ovar^t_j \nrightarrow E$) then the fact that we ignore the inter-explicit recurrence does not allow for the gradient to go from a neuron $k$ that is connected to readout neurons across the synapse $kj$ and affect the other synapses $ji$ (see Fig. \ref{fig:eprop}B, cyan line). Therefore, for every neuron whose synapses we want to learn, we need to connect it directly to readout neurons. As conclusion, this approximation does not work for architectures with a feed-forward part, since only the synapses of the last layer could be learned. This is a case where RTRL (and BPTT) can learn but symmetric e-prop cannot.

\subsection{Read-out neurons and filtering}

\begin{figure}
\includegraphics[width=\textwidth]{figures/Ron.png} 
\caption{Computational graph for A) implicit recurrence gradients in read-out neurons B) computation of \smash{$\cdv{\loss}{ \ovar^t_j}$}.}
\label{fig:Ron}
\end{figure}

Looking at the computation of \smash{$\cdv{\loss}{ \ovar^t_j}$} (see Fig \ref{fig:Ron}B):
 
\begin{equation}\label{eqpepz}
    \cdv{\loss}{ \ovar^t_j} = \sum_k \dv{E}{y^t_k}\cdv{ y^t_k}{ \ovar^t_j}
\end{equation}

For the particular structure of an LSNN with read-out neurons being LIF and the output considered its voltage $y^t_k$ (see Eq. \ref{eqron}), we get that \smash{$\dv{E}{y^t_k}$} is a non-causal gradient. 
 
We can do an equivalent trick as we did with the implicit recurrence in Section \ref{sect:ReexImplicitRec}. To do this, we first write a recursive definition (by the readout neuron's implicit recurrence) of the gradient \smash{$\dv{E}{y^t_k}$} (Fig \ref{fig:Ron}A):

\begin{equation}
    \dv{E}{y^t_k} = \cdv{\loss}{ y^t_k} + \dv{E}{y^{t+1}_k} \cdv{ y^{t+1}_k}{ y^t_k}
\end{equation}
And we plug it in Eq. \ref{eqpepz} to obtain:

\begin{equation}
\begin{split}
    \cdv{\loss}{ \ovar^{t'}_j} =& \sum_{k} \left( \cdv{\loss}{ y^{t'}_k} + \dv{E}{y^{t'+1}_k}\cdv{ y_k^{t'+1}}{ y_k^{t'}} \right) \cdv{ y^{t'}_k}{ \ovar^{t'}_j} = \\
    =&\sum_{k} \left( \cdv{\loss}{ y^{t'}_k} + \left( \cdv{\loss}{ y^{t'+1}_k} + (\dotsi) \cdv{ y_k^{t'+2}}{ y_k^{t'+1}} \right) \cdv{ y_k^{t'+1}}{ y_k^{t'}} \right) \cdv{ y^{t'}_k}{ \ovar^t_j} = \\
    =&\sum_{k}\sum_{t \geq t'} \cdv{\loss}{ y^t_k} \cdv{ y^t_k}{ y^{t-1}_k} \dotsi \cdv{ y^{t'+1}_k}{ y^{t'}_k} \cdv{ y^{t'}_k}{ \ovar^{t'}_j}
\end{split}
\end{equation}

If we plug it in the equation of symmetric e-prop Eq. \ref{eqseprop}, we can make a change of indices to make it causal as follows:

\begin{equation}
\begin{split}
    \Delta W^{rec}_{ji} &= - \eta \sum_k \sum_{t', t \geq t'} \cdv{\loss}{ y^t_k} \cdv{ y^t_k}{ y^{t-1}_k} \dotsi \cdv{ y^{t'+1}_k}{ y^{t'}_k} \cdv{ y^{t'}_k}{ \ovar^{t'}_j} e^{t'}_{ji} =\\
    &= - \eta \sum_{k,t} \cdv{\loss}{ y^t_k} \sum_{t' \leq t} \cdv{ y^t_k}{ y^{t-1}_k} \dotsi \cdv{ y^{t'+1}_k}{ y^{t'}_k} \cdv{ y^{t'}_k}{ \ovar^{t'}_j} e^{t'}_{ji} 
\end{split}
\end{equation}

From here using \smash{$\cdv{ y^t_k}{ y^{t-1}_k} = \kappa$} and \smash{$\cdv{ y^{t}_k}{ \ovar^{t}_j} = W^{out}_{kj}$} (see Eq. \ref{eqron}) we conclude:

\begin{equation}
\begin{split}
    \Delta W^{rec}_{ji} = - \eta \sum_{k,t} W^{out}_{kj} \cdv{\loss}{ y^t_k} \sum_{t' \leq t} \kappa^{t'-t} e^{t'}_{ji} 
\end{split}
\end{equation}

Finally, we define the \emph{low-pass filter operator} for any time series $x$ as: 

\begin{equation}
    \mathcal{F}_{\alpha}(x^t) = \alpha\mathcal{F}_{\alpha}(x^{t-1}) + x^t
\end{equation}
and $\mathcal{F}_{\alpha}(x^0) = x^0$. And we define the \emph{learning signal} $L^t_j$ as:

\begin{equation}
    L^t_j = \sum_k W^{out}_{kj} \cdv{\loss}{ y^t_k}
\end{equation}

With this we arrive to the final equation for \emph{symmetric e-prop readout}:

\begin{equation}\label{eqsepropron}
    \Delta W^{rec}_{ji} = - \eta \sum_{t} L^t_j \mathcal{F}_{\kappa}(e^t_{ji})
\end{equation}

\subsection{Learning signals}

Learning signals in the literature are of the general form:

\begin{equation}
    L^t_j = \sum_k B_{jk} f(y^t_k, y^{*,t}_k)
\end{equation}

In our case, $B_{jk} = W^{out}_{kj}$ and $f(y^t_k, y^{*,t}_k) = \cdv{\loss}{ y^t_k}$.

An important point to make here is that learning signals are not local. We can imagine that there are $k$ comparator neurons that compute $f(y^t_k, y^{*,t}_k)$ and send a signal with a connection weight $B_{jk}$ to neuron $j$ (see Fig. \ref{fig:learning}). However this connectivity from a ``teacher module'' to each of the neurons (note that not to each of the synapses), is minimum to be able to evaluate how the network is performing. We will call e-prop local (even though this connectivity is required) since no connections inside the RSNN between neurons and synapses are required. As we will discuss in Section \ref{sect:learningsignal}, it is not so biologically implausible to think about such a global custom signal. 

\begin{figure}
\includegraphics[width=\textwidth]{figures/learning.png} 
\caption{Diagram of the learning signal $L^t_j$ where the intensity of the signals are written as labels to the edges.}
\label{fig:learning}
\end{figure}


\subsection{Symmetric e-prop family}

Now, we are going to look at particular learning rules that arrive from considering particular loss functions $E$.

\subsubsection{Regression}
\label{sect:regression}

Consider regression, where we want the activity of the readout neurons $y_1^t, ..., y_k^t$ to match a given target activity $y^{*,t}_1,...,y^{*,t}_k$ at all times. We can define the loss function as the MSE (Mean Square Error) as follows:

\begin{equation}
    E = \frac{1}{2} \sum_{t,k} (y^t_k - y^{*,t}_k)^2
\end{equation}

Then we have 
\begin{equation}
    \cdv{\loss}{ y^{t}_k} = (y^{t}_k - y^{*,t}_k)
\end{equation}

Introducing this into Eq. \ref{eqsepropron} we obtain the equation for \textbf{regression symmetric e-prop}:

\begin{equation}
\begin{split}
    \Delta W^{rec}_{ji} = -\eta \sum_{t} L^t_j \mathcal{F}_{\kappa}(e^t_{ji})  \\
    L^t_j =  \sum_{k} W^{out}_{kj}(y^t_k- y^{*,t}_k)
\end{split}
\end{equation}

\subsubsection{Classification}
Consider the task of classification with $K$ possible classes. At each time step we have a one-hot encoded vector $\pi^{*,t}_1, ... , \pi^{*,t}_K$ ($\pi^{*,t}_k = 1$ if the input at time $t$ belongs to class $k$ and $= 0$ otherwise). From our readout neurons $y^t_1,...,y^t_k$ we compute the predicted probability that the input at time $t$ belongs to class $k$ as $\pi^t_k = softmax_k(y_1^t,...,y_K^t)$. For this task we can use the CE (Cross-Entropy) error as loss function:

\begin{equation}
    E = -\sum_{t,k} \pi^{*,t}_k \log\pi^t_k
\end{equation}

Then, in the same way as before, we arrive at the \textbf{classification symmetric e-prop}:

\begin{equation}
\begin{split}
    \Delta W^{rec}_{ji} = -\eta \sum_{t} L^t_j \mathcal{F}_{\kappa}(e^t_{ji})  \\
    L^t_j =  \sum_{k} W^{out}_{kj}(\pi^t_k- \pi^{*,t}_k)
\end{split}
\end{equation}

\subsubsection{Reinforcement learning}
Consider the task of RL (Reinforcement Learning). The encoding of the policy of the agent is encoded by the readout neurons $\pmb{y}^t = y_1^t,...,y_k^t$. This means that the agent will take action $k$ at time $t$ with probability $\pi_k^t = \pi(a^t = k|\pmb{y}^t) = softmax_k(y_1^t,...,y_k^t)$. The objective is to maximise the expected return at time $t=0$ ($\mathbb{E}[R^0]$) where the return is defined as $R^t = \sum_{t' \geq t} \gamma^{t'-t}r^{t'}$ with $r^t$ a reward obtained at time $t$ and $\gamma \leq 1$ a time discount factor. There is also one extra readout neuron $y^t_V$ that represents the value function $V^t$, which predicts the value of the expected return at each time step ($V^t \approx  \mathbb{E}[R^t]$). With this, we define the actor-critic loss function as:

\begin{equation}
    E = E_{\pi} +c_VE_V
\end{equation}
where ``the actor'' $E_\pi = -\sum_{t} R^t log \pi(a^t|\pmb{y}^t)$ measures how good the policy $\pi$ is, ``the critic'' $E_V = \sum_{t} \frac{1}{2}(R^t - V^t)^2$ measures how good the estimator $V^t$ is, and $c_V$ is a hyperparameter.

Then, the \textbf{RL symmetric e-prop} is:

\begin{equation}
\begin{split}
    \Delta W^{rec}_{ji} = - \eta \sum_t \delta^t \mathcal{F}_{\gamma}(L^t_j \mathcal{F}_{\kappa} (e^t_{ji})) \\
    L^t_j = -c_V W^{out}_{Vj} + \sum_k W^{out}_{kj}(\pi^t_k - \pmb{1}_{a^t=k})
\end{split}
\end{equation}
where $\delta^t = r^t + \gamma^{t+1}-V^t$ is the temporal difference error that can be computed in a causal manner with the introduction of appropriate extra eligibility traces \cite{Sutton1999}. Here the expression of e-prop algorithm is more convoluted since we require a more complex structure for the read-out neurons.

\section{Adaptive and Random e-prop}

We have stated that we accept the learning signal to be non-local since it is not so biologically implausible. However, a big problem is weight sharing: the intensity of the learning signal from comparator $k$ to neuron $j$ is modulated by the same weight as that from neuron $j$ to readout neuron $k$: i.e. $B_{jk} = W^{out}_{kj}$ (see Fig. \ref{fig:Ron}). Therefore, both connections need to have the same strength all the time. 

This is why the algorithm family is named ``symmetric''. The following types of e-prop try to address this issue.

\subsection{Adaptive e-prop}

One solution is to initialise randomly the comparator neurons' weights $B_{jk}$ and then modify them accordingly to the readout weights:

\begin{equation}
    \Delta W^{out}_{kj} = \Delta B_{jk}
\end{equation}

This still requires a high coordination and some biological mechanism to keep them both synchronised but it is not as restrictive as in symmetric e-prop where $B_{jk} = W^{out}_{kj}$. The family of learning rules that are formed with this approximation of the learning signal are called \textbf{adaptive e-prop family}.

\subsection{Random e-prop}

Another further simplification is to initialise randomly $B_{jk}$ and fix its value. This is a further approximation of symmetric e-prop which is already an approximation of RTRL. It does, however, work well in practice. And does not need any kind of weight sharing between $B_{jk}$ and $W^{out}_{kj}$.

Furthermore, we solve a problem presented in Section \ref{sect:FFrest}, where we stated that if a neuron is not directly connected to a readout neuron, then e-prop algorithms would not let its synapses to learn. In this case, since the weight of the learning signal is disconnected from the weight between each neuron and a readout neuron, we can assign random $B_{jk}$ to neurons $j$ for which $W^{out}_{jk}$ does not exist. This lifts the restriction we had presented of architectures not being able to have a feed-forward part.

The family of learning rules that are formed with this approximation of the learning signal are called \textbf{random e-prop family}.


\section{Complexity}

e-prop solves the problem of RTRL of being local (except for the learning signal) while being causal. Also, it is less computational and memory expensive than RTRL. Computational and memory complexity is not only important in practical applications, but it is also important for biological plausibility since we expect evolution to optimise the two. Given $n$ neurons simulated $T$ time steps with $p$ synapses, we see the complexities of the different models in Table \ref{table:com} \cite{Bellec2020, Zenke2020}:

\begin{table}[ht]
\centering
\begin{tabular}{@{\extracolsep{30pt}}lcc}
\toprule   
{} & \multicolumn{2}{c}{Complexity}\\
 \cmidrule{2-3} 
 Algorithm & Computation & Memory \\ 
\midrule
BPTT & $O(n^2T)$ & $O(nT)$  \\ 
RTRL & $O(n^4T)$ & $O(np)$ \\ 
e-prop & $O(n^2T)$ & $O(p)$ \\ 
\bottomrule
\end{tabular}
\caption{Computational and memory complexity of BPTT, RTRL and e-prop.} 
\label{table:com}
\end{table}

RTRL has a computational complexity of $O(n^4T)$ in total ($O(n^4)$ per time step). This complexity is prohibitive in comparison to BPTT which belongs to $O(n^2T)$ in total ($O(n^2)$ per time step, even though since it is not causal it cannot be implemented online and so there is no per time step computation). e-prop has a computational complexity of $O(n^2T)$ in total (and indeed now $O(n^2)$ per time step), so is as good as BPTT.

With regards to memory complexity, BPTT is $O(nT)$ (the variables' values of each neuron at each time step, since it is not local), usually much less than the memory requirements of RTRL which is $O(np)$ (the recurrent elegibility trace of each neuron for each synapse). Since normally we connect all neurons to all neurons this means that $p = n^2$ and that the memory cost is $O(n^3)$, very prohibitive. e-prop has a memory complexity of $O(p)$ (the elegibility trace of each synapse). It is therefore $O(n^2)$ for $p = n^2$. This is not as good as BPTT but way better than RTRL.

The main drawback of e-prop is that is an approximation of the gradient and, therefore, in theory, it should take more iterations to converge to an optimal value. We see however that in practical examples the increase in the number of iterations is not prohibitive \cite{Bellec2019, Bellec2020}.
